Hypergraph Acyclicity Revisited

The notion of graph acyclicity has been extended to several different notions of hypergraph acyclicity, in increasing order of generality: gamma acyclicity, beta acyclicity, and alpha acyclicity, that have met a great interest in many fields. We prove the equivalence between the numerous characterizations of each notion with a new, simpler proof, in a self-contained manner. For that purpose, we introduce new notions of alpha, beta and gamma leaf that allow to define new "rule-based" characterizations of each notion. The combined presentation of the notions is completed with a study of their respective closure properties. New closure results are established, and alpha, beta and gamma acyclicity are proved optimal w.r.t. their closure properties.

==> bar.tex <==
\makeatletter
\newsavebox\myboxA
\newsavebox\myboxB
\newlength\mylenA

\newcommand*\xoverline[2][0.75]{%
    \sbox{\myboxA}{$\m@th#2$}%
    \setbox\myboxB\null% Phantom box
    \ht\myboxB=\ht\myboxA%
    \dp\myboxB=\dp\myboxA%
    \wd\myboxB=#1\wd\myboxA% Scale phantom
    \sbox\myboxB{$\m@th\overline{\copy\myboxB}$}%  Overlined phantom
    \setlength\mylenA{\the\wd\myboxA}%   calc width diff
    \addtolength\mylenA{-\the\wd\myboxB}%
    \ifdim\wd\myboxB<\wd\myboxA%
       \rlap{\hskip 0.5\mylenA\usebox\myboxB}{\usebox\myboxA}%
    \else
        \hskip -0.5\mylenA\rlap{\usebox\myboxA}{\hskip 0.5\mylenA\usebox\myboxB}%
    \fi}
\makeatother



==> beta.tex <==
\shorthandoff{;:!?}\xygraph{
	!{<0cm,0cm>;<0.75cm,0cm>:<0cm,0.75cm>::}
	!{(-0.25, 0.0)}="Nm0_25__0_0"
	!{(0.5, 0.25)}="N0_5__0_25"
	!{(0.0, -0.5)}="N0_0__m0_5"
	!{(0.0, 0.5)}="N0_0__0_5"
	!{(-1.2675, 0.0)}="Nm1_2675__0_0"
	!{(0.5, -0.25)}="N0_5__m0_25"
	!{(-0.5175, -0.25)}="Nm0_5175__m0_25"
	!{(-1.5, 0.0)}="Nm1_5__0_0"
	!{(-0.5, 0.25)}="Nm0_5__0_25"
	!{(0.25, 0.0)}="N0_25__0_0"
	!{(1.5, 0.0)}="N1_5__0_0"
	!{(1.25, 0.0)}="N1_25__0_0"
	!{(-1.0, 0.0)}*+{x}="Nm1_0__0_0"
	!{(0.0, 0.0)}*+{y}="N0_0__0_0"
	!{(1.0, 0.0)}*+{z}="N1_0__0_0"
	"Nm0_5__0_25"-@`{(0.25, 0.25)}"N0_25__0_0"
	"N0_25__0_0"-@`{(0.25, -0.25)}"Nm0_5175__m0_25"
	"Nm0_5175__m0_25"-@`{(-1.285, -0.25)}"Nm1_2675__0_0"
	"Nm1_2675__0_0"-@`{(-1.25, 0.25)}"Nm0_5__0_25"
	"N0_5__0_25"-@`{(1.25, 0.25)}"N1_25__0_0"
	"N1_25__0_0"-@`{(1.25, -0.25)}"N0_5__m0_25"
	"N0_5__m0_25"-@`{(-0.25, -0.25)}"Nm0_25__0_0"
	"Nm0_25__0_0"-@`{(-0.25, 0.25)}"N0_5__0_25"
	"N0_0__0_5"-@`{(1.5, 0.5)}"N1_5__0_0"
	"N1_5__0_0"-@`{(1.5, -0.5)}"N0_0__m0_5"
	"N0_0__m0_5"-@`{(-1.5, -0.5)}"Nm1_5__0_0"
	"Nm1_5__0_0"-@`{(-1.5, 0.5)}"N0_0__0_5"
}

==> gamma.tex <==
\shorthandoff{;:!?}\xygraph{
	!{<0cm,0cm>;<0.75cm,0cm>:<0cm,0.75cm>::}
	!{(0.0, 0.75)}="N0_0__0_75"
	!{(-0.34641016151377546, 0.0)}="Nm0_346410161514__0_0"
	!{(0.0, -0.75)}="N0_0__m0_75"
	!{(0.25, 0.0)}="N0_25__0_0"
	!{(0.6062177826491071, -0.55)}="N0_606217782649__m0_55"
	!{(-0.25, 0.0)}="Nm0_25__0_0"
	!{(0.6062177826491071, 0.55)}="N0_606217782649__0_55"
	!{(0.0, -0.5)}*+{z}="N0_0__m0_5"
	!{(0.8660254037844386, 0.0)}*+{t}="N0_866025403784__0_0"
	!{(0.0, 0.5)}*+{y}="N0_0__0_5"
	"N0_606217782649__m0_55"-@`{(1.5588457268119895, 0.0)}"N0_606217782649__0_55"
	"N0_606217782649__0_55"-@`{(-0.34641016151377546, 1.1)}"Nm0_346410161514__0_0"
	"Nm0_346410161514__0_0"-@`{(-0.34641016151377546, -1.1)}"N0_606217782649__m0_55"
	"N0_0__m0_75"-@`{(0.25, -0.75)}"N0_25__0_0"
	"N0_25__0_0"-@`{(0.25, 0.75)}"N0_0__0_75"
	"N0_0__0_75"-@`{(-0.25, 0.75)}"Nm0_25__0_0"
	"Nm0_25__0_0"-@`{(-0.25, -0.75)}"N0_0__m0_75"
}

==> graph.tex <==
\shorthandoff{;:!?}\xygraph{
	!{<0cm,0cm>;<0.75cm,0cm>:<0cm,0.75cm>::}
	!{(0.0, 1.0)}="N0_0__1_0"
	!{(0.5, 0.5)}="N0_5__0_5"
	!{(-0.5, 0.0)}="Nm0_5__0_0"
	!{(-2.0, 0.0)}="Nm2_0__0_0"
	!{(0.5, -0.5)}="N0_5__m0_5"
	!{(0.5, 0.0)}="N0_5__0_0"
	!{(-0.5, 0.5)}="Nm0_5__0_5"
	!{(2.0, 0.0)}="N2_0__0_0"
	!{(-0.5, -0.5)}="Nm0_5__m0_5"
	!{(0.0, -1.0)}="N0_0__m1_0"
	!{(1.5, 0.0)}="N1_5__0_0"
	!{(-1.5, 0.0)}="Nm1_5__0_0"
	!{(-1, 0)}*+{x}="Nm1__0"
	!{(0, 0)}*+{y}="N0__0"
	!{(1, 0)}*+{z}="N1__0"
	"Nm0_5__0_5"-@`{"N0_5__0_5"}"N0_5__0_0"
	"N0_5__0_0"-@`{"N0_5__m0_5"}"Nm0_5__m0_5"
	"Nm0_5__m0_5"-@`{(-1.5, -0.5)}"Nm1_5__0_0"
	"Nm1_5__0_0"-@`{(-1.5, 0.5)}"Nm0_5__0_5"
	"N0_5__0_5"-@`{(1.5, 0.5)}"N1_5__0_0"
	"N1_5__0_0"-@`{(1.5, -0.5)}"N0_5__m0_5"
	"N0_5__m0_5"-@`{"Nm0_5__m0_5"}"Nm0_5__0_0"
	"Nm0_5__0_0"-@`{"Nm0_5__0_5"}"N0_5__0_5"
	"N0_0__1_0"-@`{(2.0, 1)}"N2_0__0_0"
	"N2_0__0_0"-@`{(2.0, -1)}"N0_0__m1_0"
	"N0_0__m1_0"-@`{(-2.0, -1)}"Nm2_0__0_0"
	"Nm2_0__0_0"-@`{(-2.0, 1)}"N0_0__1_0"
}

==> headers.tex <==

%\usepackage{blindtext}

\makeatletter
\if@twoside
  \def\ps@headings{%
      \let\@oddfoot\@empty\let\@evenfoot\@empty       % No footer
      \def\@evenhead{%\small%
		{\sffamily\bfseries\color{grisf}\thepage}
		{\sffamily\fontseries{sbc}\selectfont\color{grisf}\hfil\leftmark}
		}%   % Header on even pages small
      \def\@oddhead{%\small
		\sffamily\fontseries{sbc}\selectfont\color{grisf}%
		\rightmark\hfil
		{\sffamily\bfseries\color{grisf}\thepage}
		}%   % Header on  odd pages small
      \let\@mkboth\markboth
    \def\chaptermarkS##1{%
      \markboth{%\scshape%                             % Chapters in Header capitalized
		\sffamily\fontseries{sbc}\selectfont\color{grisf}
        ##1}{}}%
    \def\chaptermark##1{%
      \markboth{%\scshape%                             % Chapters in Header capitalized
		\sffamily\fontseries{sbc}\selectfont\color{grisf}
        \ifnum \c@secnumdepth >\m@ne
            \@chapapp\ \thechapter. \ %
        \fi
        ##1}{}}%
    \def\sectionmark##1{%
      \markright{%\scshape%                            % Sections in Header capitalized
		\sffamily\fontseries{sbc}\selectfont\color{grisf}
       \ifnum \c@secnumdepth >\z@
         \thesection. \ %
       \fi
       ##1}}}
\else
  \def\ps@headings{%
    \let\@oddfoot\@empty
    \def\@oddhead{\small\rightmark\hfil\thepage}%      % Header font small
    \let\@mkboth\markboth
    \def\chaptermark##1{%
      \markright{\scshape%                             % Chapters in Header capitalized
        \ifnum \c@secnumdepth >\m@ne
            \@chapapp\ \thechapter. \ %
        \fi
        ##1}}}
\fi
\makeatother
\aliaspagestyle{part}{empty}

\makepagestyle{mychapter}
\makeevenfoot{mychapter}{}{\sffamily\bfseries\color{grisf}\thepage}{}
\makeoddfoot{mychapter}{}{\sffamily\bfseries\color{grisf}\thepage}{}
\aliaspagestyle{chapter}{mychapter}

%\makepagestyle{myheadings}
%\copypagestyle{myheadings}{headings}
%\makeoddhead{myheading}{}{\color{grisf}{\textbf{\thepage}}}{}

\pagestyle{headings}
%\usepackage{fancyhdr}
%\renewcommand{\headrulewidth}{0.4pt}
%\renewcommand{\footrulewidth}{0.4pt}


%%% typesets the TITLE page
\newcommand{\thetitlepage}{{%
\clearpage
\thispagestyle{empty}
\centering
\vspace*{-\toptafiddle}
\asutitle \\ by \\ \asuauthor
\vfill
{\SingleSpace
A \asudoctype\ Presented in Partial Fulfillment \\
of the Requirements for the Degree \\
\asudegree\par}
\vfill
ARCHIBALD SMYTHE UNIVERSITY \\
\asugraddate
\par
\enlargethispage{\bottafiddle}
\clearpage}}




==> nestex.tex <==
\shorthandoff{;:!?}\xygraph{
	!{<0cm,0cm>;<0.75cm,0cm>:<0cm,0.75cm>::}
	!{(-0.09999999999999981, 0.762102355330306)}="Nm0_1__0_76210235533"
	!{(1.1, 0.762102355330306)}="N1_1__0_76210235533"
	!{(-0.7100000000000001, 0.29444863728670956)}="Nm0_71__0_294448637287"
	!{(-0.21000000000000002, 0.5715767664977295)}="Nm0_21__0_571576766498"
	!{(-0.10999999999999988, 1.3336791218280357)}="Nm0_11__1_33367912183"
	!{(0.6099999999999997, -0.46765371804359707)}="N0_61__m0_467653718044"
	!{(-0.10000000000000014, -0.7621023553303061)}="Nm0_1__m0_76210235533"
	!{(1.7100000000000002, 0.29444863728670906)}="N1_71__0_294448637287"
	!{(1.21, 0.5715767664977291)}="N1_21__0_571576766498"
	!{(1.0999999999999999, -0.7621023553303061)}="N1_1__m0_76210235533"
	!{(0.39, -0.46765371804359684)}="N0_39__m0_467653718044"
	!{(1.11, 1.3336791218280353)}="N1_11__1_33367912183"
	!{(0.2, 0.1)}*+{x}="N0_2__0_1"
	!{(0.8, 0.1)}*+{y}="N0_8__0_1"
	!{(0.5, 0.6928203230275509)}*+{z}="N0_5__0_692820323028"
	!{(1.5, 0.8660254037844386)}*+{a}="N1_5__0_866025403784"
	!{(-0.5, 0.8660254037844386)}*+{b}="Nm0_5__0_866025403784"
	!{(0.5, -0.8660254037844386)}*+{c}="N0_5__m0_866025403784"
	"Nm0_1__0_76210235533"-@`{(-0.7, 0.0)}"Nm0_1__m0_76210235533"
	"Nm0_1__m0_76210235533"-@`{(0.49999999999999967, -1.5242047106606122)}"N1_1__m0_76210235533"
	"N1_1__m0_76210235533"-@`{(1.7, 0.0)}"N1_1__0_76210235533"
	"N1_1__0_76210235533"-@`{(0.5000000000000003, 1.524204710660612)}"Nm0_1__0_76210235533"
	"N1_21__0_571576766498"-@`{(0.8500000000000001, 1.4722431864335457)}"Nm0_11__1_33367912183"
	"Nm0_11__1_33367912183"-@`{(-1.0699999999999998, 1.195115057222526)}"Nm0_71__0_294448637287"
	"Nm0_71__0_294448637287"-@`{(-0.3500000000000003, -0.6062177826491069)}"N0_61__m0_467653718044"
	"N0_61__m0_467653718044"-@`{(1.5699999999999996, -0.32908965343808727)}"N1_21__0_571576766498"
	"N0_39__m0_467653718044"-@`{(1.35, -0.606217782649107)}"N1_71__0_294448637287"
	"N1_71__0_294448637287"-@`{(2.0700000000000003, 1.195115057222525)}"N1_11__1_33367912183"
	"N1_11__1_33367912183"-@`{(0.15000000000000002, 1.4722431864335457)}"Nm0_21__0_571576766498"
	"Nm0_21__0_571576766498"-@`{(-0.5700000000000001, -0.3290896534380867)}"N0_39__m0_467653718044"
}
